RobustSleepNet: Transfer learning for automated sleep staging at scale

Sleep disorder diagnosis relies on the analysis of polysomnography (PSG) records. As a preliminary step of this examination, sleep stages are systematically determined. In practice, sleep stage classification relies on the visual inspection of 30-second epochs of polysomnography signals. Numerous automatic approaches have been developed to replace this tedious and expensive task. Although these methods demonstrated better performance than human sleep experts on specific datasets, they remain largely unused in sleep clinics. The main reason is that each sleep clinic uses a specific PSG montage that most automatic approaches cannot handle out-of-the-box. Moreover, even when the PSG montage is compatible, publications have shown that automatic approaches perform poorly on unseen data with different demographics. To address these issues, we introduce RobustSleepNet, a deep learning model for automatic sleep stage classification able to handle arbitrary PSG montages. We trained and evaluated this model in a leave-one-out-dataset fashion on a large corpus of 8 heterogeneous sleep staging datasets to make it robust to demographic changes. When evaluated on an unseen dataset, RobustSleepNet reaches 97% of the F1 of a model explicitly trained on this dataset. Hence, RobustSleepNet unlocks the possibility to perform high-quality out-of-the-box automatic sleep staging with any clinical setup. We further show that finetuning RobustSleepNet, using a part of the unseen dataset, increases the F1 by 2% when compared to a model trained specifically for this dataset. Therefore, finetuning might be used to reach a state-of-the-art level of performance on a specific population.

==> backup/backup.tex <==


The average confusion matrix per dataset for the three setups is reported in Fig.\ref{figure:confusion_matrix}. The confusion matrix of each dataset is computed, and we average each of the cells across the datasets. The three setups show similar error distribution and most of the errors are between WAKE and N1, N1 and N2, N1 and REM and N2 and N3.


 \begin{figure*}[t]
\vspace{-1em}
    \begin{center}
    \includegraphics[width=\linewidth]{figures/confusion_matrices.png} 
    \caption{Confusion matrices of RobustSleepNet in the 3 setups. The confusion matrices are computed each of the dataset and averaged to ensure equal weights between the datasets.}
    \label{figure:confusion_matrix}
    \end{center}
    \vspace{-1em}
\end{figure*}

\begin{figure}
\vspace{-1em}
    \begin{center}
    \includegraphics[width=\linewidth]{figures/scorers_transfer.png} 

    \caption{Epoch-wise F1 of RobustSleepNet in DT when trained on DODO and DODH depending on which annotations are used as the ground truth. Consensus denotes the setup when the consensus of the 5 scorers are used as ground truth for training. Average scorer denotes the average of the five models, each of which are trained on annotations from a single scorer.}
    \label{figure:scorers_transfer}
    \end{center}
    \vspace{-1em}
\end{figure}

==> tables/back/dataset_description_back.tex <==
\newcolumntype{L}{>{\centering\arraybackslash}m{3cm}}
\newcolumntype{X}{>{\centering\arraybackslash}m{4cm}}
\begin{table*}[t]
\centering

\begin{tabular}{l|lLllllXl} 

 \hline
Dataset  & Nights & Channels used & Male (\%) & Age & BMI & AHI & Other disorders & TST (min) \\
 \hline
CAP & 106 & 2xEEG, EOG & 61& $45.2 \pm 19.6$ & - & - & NFLE(40), PLM(10), RBD(22), Bruxism(2), Narcolepsy(5), Insomnia(9)  & 410 \\
DODH & 25 & 12xEEG, 2xEOG, EMG & 76.0 & $35.3 \pm 7.5$ & $23.8 \pm 3.4 $ & $\leq 5$ & No & 427 \\
DODO & 55 & 8xEEG, 2xEOG, EMG & 63.6 &$45.6 \pm 16.5$  & $29.6 \pm 6.4$  & $18.5 \pm 16.2$ & No & 387 \\
MASS SS1 & 53 & 2xEEG, EEG/EOG, EOG, EMG & 64.1 &$63.6 \pm 5.3$ & - & $\leq 20$ & No & 426 \\
MASS SS3 & 62 & 2xEEG, EEG/EOG, EOG, EMG & 45.2 &$42.5 \pm 18.9$ & -  & $\leq 10$ & No & 426 \\
MESA & 2053 & 3xEEG, 2xEOG, EMG & 53.5 & $69.6 \pm 9.2$ & - &  $16.1 \pm 13.7$ & Not reported & 359\\
MROS & 586 & 5xEEG, EOG, 2xEMG  & 100 & $81.0 \pm 4.4$& $26.9	\pm 3.9$ & $17.1 \pm 15.6$  & Parkinson(16), Alzheimer(15), Narcolepsy(1), RLS(25), PLM(11) & 341 \\
SC 39 & 39 & 2xEEG, EOG & 50.0  & $28.65 \pm 2.9$ & - & - & No & 436 \\
SC 153 & 153 & 2xEEG, EOG & 48.6  & $58.8 \pm 22.1 $ & - & - & No & 423 \\
ST & 44 & 2xEEG, EOG & 31.8 &$40.2 \pm 18$  & - & - & Difficulties falling asleep(44), Nights recorded afetr Temazepam intakes(22) & 434 \\
SleepEDF & 197 & 2xEEG, EOG & 56 & $54.7 \pm 22.6 $  & - & - & No & 426 \\
SHHS & 2651 & 2xEEG, 2xEOG, EMG & 45.6 & $68.3 \pm 10.5$ & $28.3 \pm 5.1$  & $14.6 \pm 12.0$ & Narcolepsy(9), Insomnia(46), PLM(56)  & 371 \\

 \hline
 
\end{tabular}
\caption{Datasets demographics. All values are averaged across subjects. When AHI is reported, we report the mean AHI and its deviation, if AHI is used as an exclusion criterion, we report this criterion, otherwise, the cell is left blank. We report sleep disorder and the number subjects said to have been diagnosed for in parenthesis, hence not all pathologies may not reported. \\ \small{NFLE: Nocturnal frontal lobe epilepsy. PLM: Periodic leg movements. RBD: REM behavior disorder. RLS: Restless legs syndrom}}

\label{tab:dataset_desctiption}
\vspace{-1 em}
\end{table*}

==> tables/back/full_model_old.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{|c|c| c c| c c |c c c c|c|c|c|c|} 
 \hline
  & & \multicolumn{2}{c|}{Dreem Open Datasets} & \multicolumn{2}{c|}{MASS} & \multicolumn{4}{c|}{Sleep EDF} & MROS & MESA & SHHS & CAP\\ 
 & Model  & DODO & DODH  & SS1 & SS3 & SC-39 & SC-153 & ST & Full &  &  &  & \\ 
 
 \hline
 \multirow{5}*{\rotatebox{90}{FT}} 
 & RobustSleepNet & \textbf{82.7} & \textbf{85.1} & - & 84.0  & \textbf{81.7} & \textbf{77.9} & \textbf{81.0} & \textbf{79.6} & \textbf{75.6} &  \textbf{79.5} & \textbf{80.0} & \textbf{73.8}\\
 & SeqSleepNet \cite{SingleChannelMismatch} \cite{MultipleChannelTrasnferLearning} & - & - & - & - & 80.0 & - & 77.5 &  & - & - & - & -\\
    &  SeqSleepNet \cite{MultipleChannelTrasnferLearning} & - & - & - & - & 77.7 & - & 76.7 & - & - & - & - & - \\
    &  DeepSleepNet \cite{MultipleChannelTrasnferLearning} & - & - & - & - & 79.0 & - & 77.5 & - & - & - & - & - \\
        &  KL-reg \cite{KLPersonalization} & - & - & - & - & - & 73.0  & - & - & - & - & - & - \\
   \hhline{|=|=============|} \multirow{6}*{\rotatebox{90}{DT}} & RobustNet (ours) & 79.6 & 84.6 & 76.3 & 80.6 & 80.6 & 76.0 & 80.3 & 77.2 & 72.0 &  75.2 & 75.8 & 64.8\\
& RobustSleepNet (bed-only) & - & - & - & - & 79.2 & 75.2 & 80.3 & 76.4 & - &  - & - & - \\
 &  SeqSleepNet \cite{SingleChannelMismatch} & - & - &  - & -& 74.6 & - & 75.6 & - & - & - & - & - \\
 &  SeqSleepNet \cite{MultipleChannelTrasnferLearning} & - & -& -  & - & 62.1 & - & 64.2 & - & - & - & - & - \\
 &  SimpleSleepNet \cite{guillot2019dreem} & 43.4 & 72.0 & - & - & - & - & - & - & - & - & - & - \\
    & Optimal Transport \cite{Optimal_transport_chambon} & - & - & - & 60.0 & - & - & - & - & - & - & - & - \\
    \hhline{|=|=============|} \multirow{6}*{\rotatebox{90}{LfS}}
       & RobustNet & 80.5 & 81.6 & - & 82.2 &  79.1 & 76.3 & 78.6 & 77.8 & 74.1 &  79.2 & 79.2 & 71.8 \\
    & SimpleSleepNet \cite{guillot2019dreem} & 79.4 & 82.2 & - & 84.6 & 80.5 & - & - & 79.0 & - & - & - & - \\
& DeepSleepNet \cite{guillot2019dreem} & 77.3 & 82.1 & - & \textbf{85.2} & 80.4 & - & - & 78.1 & - & - & - & - \\
    & UTime \cite{perslev2019utime}& - & - & -& - & 79.0 & 76.0 & - & - & - & - & - & 68 \\
 & CNN \cite{varela} & - & - & - & - & - & - & - &  - & -  & - & 76.0 & - \\
 & CNN \cite{Sors2018ACN} & - & - & - & - & - & - & - & - & - & - &  78.0 &  \\
 
 \hline
\end{tabular}
\centering
\caption{Epoch-wise macro-F1 of RobustNet and literatures baseline in a finetuning setup, direct trasnfer learning setup and in a standard supervised learning setting.}

\label{tab:main_table}
\vspace{-2em}
\end{table*}

==> tables/back/main_table.tex <==
\begin{table*}[t]
\centering

\scalebox{1}{%
\setlength\tabcolsep{4pt}
\begin{tabular}{|c|c| c c| c c |c c c c c c c c|c|c|c|c|} 
 \hline
 \setlength\tabcolsep{4pt}
  & & \multicolumn{2}{c|}{DOD} & \multicolumn{2}{c|}{MASS} & \multicolumn{8}{c|}{Sleep EDF} & MROS & MESA & SHHS & CAP\\ 
  \setlength\tabcolsep{4pt}
 &  & DODO & DODH  & SS1 & SS3 & \multicolumn{2}{c}{SC 39} & \multicolumn{2}{c}{SC 153}  & \multicolumn{2}{c}{ST}  & \multicolumn{2}{c|}{Full}  &  &  &  & \\ 
 
 & Model  & &  & & & (1) & (2) & (1) & (2) & (1) & (2) & (1) & (2) &  &  &  & \\ 
 \hline
 \multirow{5}*{\rotatebox{90}{FT}} 
 & RobustSleepNet & \textbf{82.7} & \textbf{85.1} & \textbf{79.7} & 84.0  & \textbf{81.7} & \textbf{81.3}  & \textbf{77.9}& \textbf{77.0}  & \textbf{81.0} & \textbf{81.0} & \textbf{79.6} & \textbf{78.3}  & \textbf{75.6} &  \textbf{79.5} & \textbf{80.0} & \textbf{73.8}\\
 & SeqSleepNet \cite{SingleChannelMismatch} \cite{MultipleChannelTrasnferLearning} & - & - & - & - & - & 80.0  & - & -& - & 77.5  & - & - & - & -& -  & - \\
    &  SeqSleepNet \cite{MultipleChannelTrasnferLearning} & - & - & - & - & - & 77.7 & -& -& -  & 76.7  & -& -& - & - & - & - \\
    &  DeepSleepNet \cite{MultipleChannelTrasnferLearning} & - & - & - & - &  - &79.0 & -& - & - & 77.5  & - & - & - & - & - & - \\
        &  KL-reg \cite{KLPersonalization} & - & - & - & - & - & - & - & 73.0   & - & - & - & - & - & - & - & - \\
   \hhline{|=|=================|} \multirow{6}*{\rotatebox{90}{DT}} & RobustSleepNet & 79.7 & 84.6 & 76.3 & 80.6 &  80.6 & 79.2 &76.0& 75.2 & 80.3 & 80.3 & 77.2 & 76.4 & 72.0 &  75.2 & 75.8 & 64.8\\
 &  SeqSleepNet \cite{SingleChannelMismatch} & - & - &  - & -& -& 74.6 & - & - & -& 75.6  & - & - & - & - & -& - \\
 &  SeqSleepNet \cite{MultipleChannelTrasnferLearning} & - & -& - & - & - & 62.1 & - & - & - & 64.2 & - & - & -& -& -& - \\
 &  SimpleSleepNet \cite{guillot2019dreem} & 43.4 & 72.0 & - & -& - & - & - & - & - & - & - & - & - & -& -& -\\
    & Optimal Transport \cite{Optimal_transport_chambon} & - & - & - & 60.0& - & - & - & - & - & - & - & - & -& -& - & - \\
    \hhline{|=|=================|} \multirow{7}*{\rotatebox{90}{LfS}}
       & RobustSleepNet & 80.5 & 81.6 & 76.7 & 82.2 &  79.1 & 78.8 & 76.3  & 75.4 & 78.6  & 77.7 & 77.8 & 77.0  & 74.1 &  79.2 & 79.2 & 71.8 \\
    & SimpleSleepNet \cite{guillot2019dreem} & 79.4 & 82.2 & - & 84.6 & 80.5 & - & -  & -   & - & - & 79.0 & -  & - & - & -  & - \\
& DeepSleepNet \cite{guillot2019dreem} & 77.3 & 82.1 & - & \textbf{85.2} & 80.4 & -  & - & - & -  & -  & 78.1 & - & - & 76.4 & - & -\\
& IITNet \cite{SEO2020102037} & &  & - & - & - & -  & - & - & -  & -  & - & - & - & - & 79.8 & -\\
 &  SeqSleepNet \cite{MultipleChannelTrasnferLearning} \cite{KLPersonalization}& - & -& - & - & - & 75.2 & 76.4 & 74.6  & - & 74.8 & - & - & -& -& -& - \\
    & UTime \cite{perslev2019utime}& - & - & -& - & 79.0 & -  & 76.0 &  -& - & - & -  & - & - & - & - & 68 \\
 & CNN \cite{varela} & - & - & - & - & - & -& - & - &  - & - & -  & -  & -  & - & 76.0 & - \\
 & CNN \cite{Sors2018ACN} & - & - & - & - & - & - &  & - & - & -  & -   & - & - & - &  78.0 &  \\
 
 \hline
\end{tabular}
}
\centering
\caption{Epoch-wise macro-F1 of RobustSleepNet and literature's baseline in a finetuning setup, direct transfer learning setup and in a standard supervised learning setting. (1) to the settings used in \cite{supratak2017deepsleepnet} \cite{perslev2019utime} and (2) corresponds to the in-bed setup described in \cite{MultipleChannelTrasnferLearning}.}

\label{tab:main_table}
\vspace{-2em}
\end{table*}

==> tables/back/scorers_f1.tex <==
\begin{table}
\centering
\newcolumntype{L}{>{\centering\arraybackslash}m{0.8cm}}
\begin{tabular}{|l|LLL|LLL|} 

 \hline
   & \multicolumn{3}{c |}{DODO} & \multicolumn{3}{c}{DODH} \\
Scorer  & Scorer F1  & Source F1 & Target F1  & Scorer F1 & Source F1 & Target F1  \\
 \hline
Scorer 1 & $71.4$ & $57.7$ & $70.7$ & $77.8$& $\textbf{61.7}$ & $75.9$\\
Scorer 2 & $73.5$ &  $65.1$& $79.0$& $80.1$ & $59.5$ & $79.1$\\
Scorer 3 & $70.6$ & $58.7$& $68.9$& $\textbf{80.8}$ & $59.8$ & $81.2$\\
Scorer 4 & $72.2$ & $64.1$ & $77.9$& $73.7$ & $53.8$ & $71.6$\\
Scorer 5 & $\textbf{75.9}$ & $65.3$ & $77.4$& $80.4$& $58.6$ & $79.3$\\
\hline
Consensus & - & $\textbf{66.2}$ & $\textbf{79.7}$ & - & $61.3$ & $\textbf{84.6}$\\
 \hline
 
\end{tabular}
\caption{Average of the subject-wise Macro F1 of the scorers against the consensus of other scorers computed as in \cite{guillot2019dreem}}
\label{tab:scorer_performances}
\vspace{-1em}
\end{table}
